Collaborative Face Experts Fusion in Video Generation: Boosting Identity Consistency Across Large Face Poses

Current video generation models struggle with identity preservation under large face poses, primarily facing two challenges: the difficulty in exploring an effective mechanism to integrate identity features into DiT architectures, and the lack of targeted coverage of large face poses in existing open-source video datasets. To address these, we present two key innovations. First, we propose Collaborative Face Experts Fusion (CoFE), which dynamically fuses complementary signals from three specialized experts within the DiT backbone: an identity expert that captures cross-pose invariant features, a semantic expert that encodes high-level visual context, and a detail expert that preserves pixel-level attributes such as skin texture and color gradients. Second, we introduce a data curation pipeline comprising three key components: Face Constraints to ensure diverse large-pose coverage, Identity Consistency to maintain stable identity across frames, and Speech Disambiguation to align textual captions with actual speaking behavior. This pipeline yields LaFID-180K, a large-scale dataset of pose-annotated video clips designed for identity-preserving video generation. Experimental results on several benchmarks demonstrate that our approach significantly outperforms state-of-the-art methods in face similarity, FID, and CLIP semantic alignment. Project page: https://rain152.github.io/CoFE/.

==> figs/cross_attn_v2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{images/cross_attn_v2.pdf}
    \vspace{-2mm}
    \caption{Extended cross-attention visualizations of different experts. }
    \label{fig:cross_attn_v2}
    % \vspace{-4mm}
\end{figure}
% The input images are from OpenHumanVid~\cite{li2025openhumanvid}.

==> figs/model_angle_band.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/angle_band_all_models.pdf}
    \caption{Statistics on face angle variations in videos generated by different models.}
    \label{fig:model_angle_band}
\end{figure}

==> figs/visual_abla_dataset.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/visual_datasets_abla.pdf}
    \caption{Visual ablation of training data processing.}
    \label{fig:visual_abla_dataset}
\end{figure}

==> figs/visual_bench.tex <==
% 第一张图
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/visual_first_frame.pdf}
    \caption{First-frame visualization of the \ourdata-Bench, featuring clear human faces and diverse scenes.}
    \label{fig:visual_bench}
\end{figure}

==> figs/visual_closesource.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{images/visual_closesource.pdf}
    \caption{Qualitative comparison with closed-source models. Our method achieves comparable visual quality.}
    \label{fig:visual_closesource}
\end{figure}

==> figs/visual_main_1.tex <==
\begin{figure*}[tbp]
    \centering
    \includegraphics[width=\linewidth]{images/visual_main_1.pdf}
    \caption{Qualitative analysis of our model and baselines (sample 1).}
    \label{fig:visual_1}
\end{figure*}

==> figs/visual_main_2.tex <==
\begin{figure*}[tbp]
    \centering
    \includegraphics[width=\linewidth]{images/visual_main_2.pdf}
    \caption{Qualitative analysis of our model and baselines (sample 2).}
    \label{fig:visual_2}
\end{figure*}

==> figs/visual_main_3.tex <==
\begin{figure*}[tbp]
    \centering
    \includegraphics[width=\linewidth]{images/visual_main_3.pdf}
    \caption{Qualitative analysis of our model and baselines (sample 3).}
    \label{fig:visual_3}
\end{figure*}

==> figs/visual_prompt.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/visual_bench_sample.pdf}
    \caption{Sample display of the \ourdata-Bench. The instructions include detailed explanations and dynamic character movements.}
    \label{fig:visual_prompt}
\end{figure}

==> figs/visual_prompt_2.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/visual_bench_sample_vip.pdf}
    \caption{Sample display of the VIP-Test. The instructions include detailed explanations and dynamic full-body motions.}
    \label{fig:visual_prompt_2}
\end{figure}

==> tables/abla_1_full.tex <==
\begin{table*}[tbp]
\renewcommand{\tabcolsep}{4pt}
\centering
\caption{Comparison of different face feature injection methods on the \ourdata-Head benchmark dataset. Our proposed \method~module still maintains significant advantages in identity preservation. In terms text relevance and visual quality, \method~remains highly competitive.}
\begin{tabular}{lccccccccc}
\hline
\hline
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Identity Preservation} & Text Relevance & \multicolumn{5}{c}{Video Quality} \\ \cline{2-3} \cline{5-9}
& FaceSim-Arc↑ & FaceSim-Cur↑ & CLIP-Score↑ & FID↓ & AQ↑ & IQ↑ & TF↑ & MS↑ \\ \hline
Wan2.1-I2V-1.3B~\cite{wan2025wan} & 0.654 & 0.656 & 29.200 & 72.322 & 0.553 & 0.66 & 0.989 & 0.993  \\
w/ ArcFace & 0.661 & 0.665 & \textbf{29.402} & 80.305 & 0.565 & 0.663 & 0.987 & 0.992 \\
w/ CLIP & 0.681 & 0.684 & 29.181 & 73.702 & 0.564 & 0.662 & 0.990 & 0.994 \\
w/ DINOv2 & 0.672 & 0.675 & 29.079 & 75.467 & 0.565 & 0.664 & 0.990 & 0.994 \\
w/ Concat & 0.732 & 0.735 & 29.143 & \textbf{63.418} & 0.567 & 0.667 & 0.990 & 0.994 \\
w/ \textbf{\method} (\textbf{Ours})& \textbf{0.770} & \textbf{0.775} & 29.125 & 63.799 & \textbf{0.570} & \textbf{0.673} & \textbf{0.990} & \textbf{0.994} \\ \hline \hline
\end{tabular}
\label{tab:abla_1_full}
\end{table*}

==> tables/abla_wan2.2.tex <==
\begin{table*}[tbp]
\renewcommand{\tabcolsep}{4pt}
\centering
\caption{Comparison of different face feature injection methods on the \ourdata-Head benchmark dataset. Our proposed \method~module still maintains significant advantages.}
\begin{tabular}{lccccccccc}
\hline
\hline
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Identity Preservation} & Text Relevance & \multicolumn{5}{c}{Video Quality} \\ \cline{2-3} \cline{5-9}
& FaceSim-Arc↑ & FaceSim-Cur↑ & CLIP-Score↑ & FID↓ & AQ↑ & IQ↑ & TF↑ & MS↑ \\ \hline
Wan2.2-TI2V-5B~\cite{wan2025wan} & 0.776 & 0.786 & 28.761 & 76.728 & 0.588 & 0.666 & 0.995 & 0.996 \\
w/ ArcFace & 0.781 & 0.792 & 28.790 & 75.842 & 0.590 & 0.663 & 0.995 & 0.996 \\
w/ CLIP & 0.792 & 0.803 & 28.822 & 74.821 & 0.590 & 0.665 & 0.996 & 0.996 \\ 
w/ DINOv2 & 0.794 & 0.806 & 28.755 & 74.707 & 0.592 & 0.668 & 0.996 & 0.996 \\
w/ Concat & 0.805 & 0.817 & 28.662 & 74.323 & \textbf{0.593} & 0.666 & 0.996 & \textbf{0.997} \\
w/ \textbf{\method} & \textbf{0.814} & \textbf{0.827} & 28.729 & \textbf{70.727} & 0.591 & \textbf{0.669} & \textbf{0.996} & 0.996 \\
\hline \hline
\end{tabular}
\label{tab:abla_2}
\end{table*}
